Hypercontractivity for Quantum Erasure Channels via Variable Multipartite Log-Sobolev Inequality

We prove an almost optimal hypercontractive inequality for products of quantum erasure channels, generalizing the hypercontractivity for classical binary erasure channels. To our knowledge, this is the first tensorization-type hypercontractivity bound for quantum channels with no fixed states. The traditional inductive arguments for classical hypercontractivity cannot be generalized to the quantum setting due to the nature of the non-commutativity of matrices. To overcome the difficulty, we establish a novel quantum log-Sobolev inequality for Bernoulli entropy, which includes the classical log-Sobolev inequality and the quantum log-Sobolev inequality as one-partite cases. To our knowledge, its classical counterpart is also unknown prior to this work. We establish a connection between our quantum log-Sobolev inequality and the hypercontractivity bound for quantum erasure channels via a refined quantum Gross' lemma, extending the analogous connection between the quantum log-Sobolev inequality and the hypercontractivity for qubit unital channels. As an application, we prove an almost tight bound (up to a constant factor) on the classical communication complexity of two-party common randomness generation assisted with erased-noisy EPR states, generalizing the tight bound on the same task assisted with erased-noisy random strings due to Guruswami and Radhakrishnan.

==> WatrousExtend2.tex <==
	\paragraph{Second part: restrict $X$ to PSD matrices}
    Our goal is to show
    $$
	    \sup_{X\in \Herm_{2^n},X\neq 0} \f{\normthree{X}_{\ep,q}}{\normthree{X}_p} \le \sup_{X\in \PSD_{2^n},X\neq 0} \f{\normthree{X}_{\ep,q}}{\normthree{X}_{p}}
	$$
	The conclusion follows immediately from
	$$
	    \normthree{X}_{\ep,q} \le \normthree{\abs{X}}_{\ep,q}, \forall X\in \Herm_{2^n}
	$$
	To show this, it is sufficient to prove for $\forall X\in \Herm_{2^n},q\in[1,2],S\subseteq[n]$, we have
	$$
	    \normthree{\tr_S \abs{X}}_q \ge \normthree{\tr_S X}_q
	$$
	
	Recall that $\diag\p{\cdot}$ denotes diagonal entries as a vector. We first show
	$$
	    \norm{\diag\p{\tr_S\abs{X}}}_q^q \ge \norm{\diag\p{\tr_S X}}_q^q
	$$
    Let $\diag\p{\abs{X}}=\p{x_1,x_2,\dots,x_{2^n}}$ and $\diag\p{X}=\p{y_1,y_2,\dots,y_{2^n}}$. Then
    \begin{align*}
        \diag\p{\tr_S\abs{X}}&=\p{\f{1}{2^{\abs{S}}}\sum_{j=1}^{2^\abs{S}} x_{2^{\abs{S}}(i-1)+j}}_{i\in\lrb{2^{n-\abs{S}}}} \\
        \diag\p{\tr_S X}&=\p{\f{1}{2^{\abs{S}}}\sum_{j=1}^{2^\abs{S}} y_{2^{\abs{S}}(i-1)+j}}_{i\in\lrb{2^{n-\abs{S}}}}
    \end{align*}
    Since both $\abs{X}-X$ and $\abs{X}+X$ are PSD matrices, we conclude that $x_k\ge\abs{y_k}$ for all $k\in [2^n]$. Therefore
    \begin{equation}\label{hyper:app:psdineq1}\begin{split}
        \norm{\diag\p{\tr_S\abs{X}}}_q^q &= \sum_{i=1}^{2^{n-|S|}}\p{\f{1}{2^{\abs{S}}}\sum_{j=1}^{2^\abs{S}} x_{2^{\abs{S}}(i-1)+j}}^q \\
        &\ge \sum_{i=1}^{2^{n-|S|}}\p{\f{1}{2^{\abs{S}}}\sum_{j=1}^{2^\abs{S}} \abs{y_{2^{\abs{S}}(i-1)+j}}}^q \\
        &\ge \sum_{i=1}^{2^{n-|S|}}\abs{\f{1}{2^{\abs{S}}}\sum_{j=1}^{2^\abs{S}} y_{2^{\abs{S}}(i-1)+j}}^q \\
        &= \norm{\diag\p{\tr_S X}}_q^q
    \end{split}\end{equation}

	Without loss of generality, we can assume $\tr_S X$ is diagonal. The following calculation shows that for any unitary matrix $V_{S^c}\in \U_{2^{n-\abs{S}}}$, we can always replace $X$ by $\p{V_{S^c}\otimes \id_{2^\abs{S}}}^\dagger X\p{V_{S^c}\otimes \id_{2^\abs{S}}}$:
	\begin{align*}
	    &\normthree{\tr_S \abs{\p{V_{S^c}\otimes \id_{2^\abs{S}}}^\dagger X\p{V_{S^c}\otimes \id_{2^\abs{S}}}}}_q = \normthree{V_{S^c}^\dagger \cdot \p{\tr_S \abs{ X}} \cdot V_{S^c}}_q = \normthree{\tr_S \abs{X}}_q \\
	    &\normthree{\tr_S \lrb{\p{V_{S^c}\otimes \id_{2^\abs{S}}}^\dagger X \p{V_{S^c}\otimes \id_{2^\abs{S}}}}}_q = \normthree{V_{S^c}^\dagger \cdot \p{\tr_S X} \cdot V_{S^c}}_q = \normthree{\tr_S X}_q
	\end{align*}
	And knowing $\tr_S X$ is diagonal, we have
	\begin{align*}
	    \normthree{\tr_S X}_q^q &= \f{1}{2^{n-\abs{S}}}\norm{ \diag\p{\tr_S X} }_q^q \\
	    &\le \f{1}{2^{n-\abs{S}}}\norm{ \diag\p{\tr_S \abs{X}} }_q^q \\
	    &\le \f{1}{2^{n-\abs{S}}}\norm{ \tr_S\abs{X} }_q^q \\
	    &=\normthree{\tr_S \abs{X}}_q^q
	\end{align*}
    where the first inequality is exactly \cref{hyper:app:psdineq1} and the second inequality follows from the fact that the eigenvalues of $\tr_S \abs{X}$ majorize its diagonal entries.

    To summarize, we conclude that
    $$
        \sup_{X\in \Herm_{2^n},X\neq 0} \f{\normthree{X}_{\ep,q}}{\normthree{X}_p} \le \sup_{X\in \PSD_{2^n},X\neq 0} \f{\normthree{X}_{\ep,q}}{\normthree{X}_{p}}
    $$
	which completes the proof of Lemma~\ref{hyper:lemma:psd}.


==> conclusion.tex <==
%%%%%%%%%%%%%% need to be refined (TODO)
We proved a hypercontractive inequality for the quantum erasure channel, which is the first hypercontractive inequality for non-unital quantum channels to our knowledge.
Our hypercontractivity for the quantum erasure channel is a natural extension
of the hypercontractivity for the classical binary erasure channel. To prove the hypercontractivity, we established a  quantum log-Sobolev inequality for Bernoulli entropy, which in interesting in its own right. As an application, we prove an almost tight lower bound on the classical communication complexity of common randomness generation assisted by erased-noisy EPR states. This work raises several open problems for future work.
\begin{enumerate}
	\item The tightness of hypercontractivity for the QEC is not clear. The hypercontractivity for classical BECs~\cite{7541363} indicates that the parameter $c$ in our result could be pushed to $1$. We leave this to future work.
		
	\item  To our knowledge, all quantum hypercontractive inequalities are only known for the channels with qubit inputs. Is it possible to establish a quantum hypercontractive inequality for qudit channels? The current approach fails even for the easy case $1\leq p\leq 2\leq q$  because the norm-compression inequality does not hold for $t\times t$ block matrices whenever $t\geq 3$ \cite{AUDENAERT2006155}. Hence, we need new techniques to establish quantum hypercontractive inequalities for qudit channels.
	
	\item The underlying distribution for quantum hypercontractive inequalities are uniform. It is interesting to consider the quantum generalization of  the classical hypercontractive inequalities over $p$-biased spaces ~\cite{O14ABF}, whose quantum counterpart is weighted non-commutative $L_p$ spaces~\cite{ricard:hal-00475221}. There have been several works investigating the hypercontractivity for quantum channels with respect to the invariant states (the generalization of stationary distributions for quantum channels)~\cite{Bardet2022-bg,beigi2020quantum}. This only implies the known result of the hypercontractivity for the quantum depolarizing channel with respect to the uniform distribution. Is it possible to establish a general quantum hypercontractive inequality in weighted non-commutative $L_p$ spaces?
	
	
	\item Log-Sobolev inequalities are a power tool to study the mixing time of a random walks on fixed graph. There are several recent works investigating the mixing time of a random on a random graph \cite{10.1214/07-AOP358,10.1214/EJP.v17-1705,rsa.20539}. The entropy in the classical multipartite log-Sobolev inequality captures the average entropy of the random subgraphs of a given graph, i.e, each vertex is deleted with probability $\ep$. Thus, it is interesting to see whether our classical log-Sobolev inequality for Bernoulli entropy can provider better analysis on the mixing time of a random walk on a random graph?
\end{enumerate}



